The language of opinion change on social media under the lens of communicative action

Which messages are more effective at inducing a change of opinion in the listener? We approach this question within the frame of Habermas' theory of communicative action, which posits that the illocutionary intent of the message (its pragmatic meaning) is the key. Thanks to recent advances in natural language processing, we are able to operationalize this theory by extracting the latent social dimensions of a message, namely archetypes of social intent of language, that come from social exchange theory. We identify key ingredients to opinion change by looking at more than 46k posts and more than 3.5M comments on Reddit's r/ChangeMyView, a debate forum where people try to change each other's opinion and explicitly mark opinion-changing comments with a special flag called "delta". Comments that express no intent are about 77% less likely to change the mind of the recipient, compared to comments that convey at least one social dimension. Among the various social dimensions, the ones that are most likely to produce an opinion change are knowledge, similarity, and trust, which resonates with Habermas' theory of communicative action. We also find other new important dimensions, such as appeals to power or empathetic expressions of support. Finally, in line with theories of constructive conflict, yet contrary to the popular characterization of conflict as the bane of modern social media, our findings show that voicing conflict in the context of a structured public debate can promote integration, especially when it is used to counter another conflictive stance. By leveraging recent advances in natural language processing, our work provides an empirical framework for Habermas' theory, finds concrete examples of its effects in the wild, and suggests its possible extension with a more faceted understanding of intent interpreted as social dimensions of language.

==> macros.tex <==
% !TEX root = main.tex

\usepackage[
  a4paper,
  hmarginratio={1:1},     % equal left and right margins
  vmarginratio={1:1},     % equal top and bottom margins
  textwidth=500pt,        % new text width
  textheight=700pt,
  heightrounded,          % always useful
  %bindingcorrection=5mm,  % binding correction
]{geometry}

\usepackage{lineno}
\usepackage[foot]{amsaddr}
\usepackage{type1cm} % type1 computer modern font
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[show]{chato-notes}
\usepackage{amsmath,amssymb}
\usepackage{mathtools} % amsmath++
\usepackage{bbm}
\usepackage{booktabs}
\usepackage{enumerate}
\usepackage{epsfig}
%\usepackage{authblk}
\usepackage{url}
\usepackage{tikz}
\usepackage{xspace}
\usepackage{balance} % to better equalize the last page
\usepackage{multirow} % multi rows for tables
\usepackage[font={bf}, tableposition=top]{caption} % captions on top for tables
\usepackage{siunitx} % \num for decimal grouping
\usepackage{microtype} % compress text
\usepackage{xfrac} % nicer slanted fractions
\usepackage[square,numbers]{natbib} % better references
\usepackage{xr-hyper} % Reference from other files (e.g. supplementary)
\usepackage{hyperref}
% \usepackage{paralist} % Inline item list
\usepackage{mdframed}

%%% THE FOLLOWING FIX IS FROM https://tex.stackexchange.com/questions/452280/xr-package-not-working-incomplete-ifx/452321#452321
% THIS IS NEEDED TO FIX PACKAGE xr-hyper
\makeatletter
\long\def\XR@test#1#2#3#4\XR@{%
  \let\XR@next\@gobbletwo
  \ifx#1\newlabel
    \let\XR@next\@firstoftwo%
  \else\ifx#1\@input
     \let\XR@next\@secondoftwo
  \fi\fi
   \XR@next{\newlabel{\XR@prefix#2}{#3}}{\edef\XR@list{\XR@list#2\relax}}%
  \ifeof\@inputcheck\expandafter\XR@aux
  \else\expandafter\XR@read\fi}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hypersetup{
    bookmarks=true,         % show bookmarks bar?
    unicode=false,          % non-Latin characters in Acrobats bookmarks
    pdftoolbar=true,        % show Acrobats toolbar?
    pdfmenubar=true,        % show Acrobats menu?
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of the page to the window
    pdftitle={My title},    % title
    pdfauthor={Author},     % author
    pdfsubject={Subject},   % subject of the document
    pdfcreator={Creator},   % creator of the document
    pdfproducer={Producer}, % producer of the document
    pdfnewwindow=true,      % links in new window
    colorlinks=true,       % false: boxed links; true: colored links
%    linkcolor=black,          % color of internal links
%    citecolor=black,        % color of links to bibliography
%    filecolor=black,      % color of file links
%    urlcolor=black           % color of external links
    linkcolor={red!50!black},
    filecolor={green!50!black},
    citecolor={green!50!black},
    urlcolor={blue!80!black},
}

\interfootnotelinepenalty=10000

%% to save space around floating bodies ( = algorithms, figures, etc.)
%\renewcommand\topfraction{0.85}
%\renewcommand\bottomfraction{0.85}
%\renewcommand\textfraction{0.1}
%\renewcommand\floatpagefraction{0.1}
%\setlength\floatsep{.05\baselineskip plus 3pt minus 4pt}
%\setlength\textfloatsep{.15\baselineskip plus 3pt minus 2pt}
%\setlength\intextsep{1.25\baselineskip plus 3pt minus 2 pt}

\newcommand{\HRule}{\rule{\linewidth}{0.1mm}}
\newcommand{\missing}{\textbf{\textcolor{red}{[missing]}}}

% Paragraphs
\newcommand{\spara}[1]{\smallskip\noindent\textbf{#1}}
\newcommand{\mpara}[1]{\medskip\noindent\textbf{#1}}
\newcommand{\para}[1]{\noindent\textbf{#1}}


\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\newcommand{\rcmv}{\texttt{r/ChangeMyView}\xspace}
\newcommand{\R}[1]{\texttt{r/#1}\xspace}
\newcommand{\cmvdelta}{\ensuremath{\Delta}\xspace}
\newcommand{\noDelta}{\overbar{\Delta}}
\newcommand{\noDeltaSet}[1]{\overline{#1_{\Delta}}}

\newcommand{\pleaseadd}[1]{\textcolor{red}{\textbf{MISSING}}}

\newcommand{\luca}[1]{\textcolor{olive}{[luca--#1]}}
\newcommand{\corrado}[1]{\textcolor{red}{[corrado--#1]}}
\newcommand{\gdfm}[1]{\textcolor{teal}{[gdfm--#1]}}
\newcommand{\fra}[1]{\textcolor{blue}{[fra--#1]}}

